Almost-Sure Reachability in Stochastic Multi-Mode System

A constant-rate multi-mode system is a hybrid system that can switch freely among a finite set of modes, and whose dynamics is specified by a finite number of real-valued variables with mode-dependent constant rates. We introduce and study a stochastic extension of a constant-rate multi-mode system where the dynamics is specified by mode-dependent compactly supported probability distributions over a set of constant rate vectors. Given a tolerance $\varepsilon > 0$, the almost-sure reachability problem for stochastic multi-mode systems is to decide the existence of a control strategy that steers the system almost-surely from an arbitrary start state to an $\varepsilon$-neighborhood of an arbitrary target state while staying inside a pre-specified safety set. We prove a necessary and sufficient condition to decide almost-sure reachability and, using this condition, we show that almost-sure reachability can be decided in polynomial time. Our algorithm can be used as a path-following algorithm in combination with any off-the-shelf path-planning algorithm to make a robot or an autonomous vehicle with noisy low-level controllers follow a given path with arbitrary precision.

==> complexity.tex <==
\begin{theorem}
  The problem of deciding almost-sure point-to-point $\varepsilon$-reachability
  is PTIME-hard.  
\end{theorem}
\begin{proof}
  In order to prove PTIME-hardness we show a reduction to the 
  almost-sure $\varepsilon$-reachability problem for \smms{} from the
  problem of deciding the alternating-graph reachability problem~\cite{Imm81}.
  An alternating-graph is a directed acyclic graph $G = (V, E \subseteq V \times
  V)$ whose vertices are partitioned into ``AND'' and ``OR'' vertices $V_\text{AND}$ and
  $V_\text{OR}$.  
  For vertices $a, b \in V$ of $G$, we say that $b$ is reachable from
  $a$ iff: 
  \begin{enumerate}
  \item $a=b$, or 
  \item $a \in V_\text{AND}$ and $b$ is reachable from all vertices $j$ such
    that $(a, j) \in E$; or
  \item $a \in V_\text{OR}$ and $b$ is reachable from some vertex $j$ such
    that $(a, j) \in E$.
  \end{enumerate}
  Immerman~\cite{Imm81} showed that alternating-graph reachability problem is
  PTIME-complete.
  We show a reduction from alternating-graph reachability problem for a graph
  $G$ to point-to-point $\varepsilon$-reachability for a \smms{} $\M_G$.
  W.l.o.g. we assume that the vertices of $G$ are numbered from $1$ to $n$. 
  Let number of variables (dimension) of $\M_G$ be equal to the number of vertices
  in $G$ and we name them $x_1, \ldots, x_n$.
  For vertices $1 \leq i, j \leq n$ we define a vector $\eta_{(i,j)}$ in the following
  manner:
  \begin{eqnarray*}
    \eta_{(i,j)}(k) =
    \begin{cases}
      -1 &\text{ if } k = i, \\
      +1 &\text{ if } k = j, \\
      0 &\text{ otherwise}.
    \end{cases}
    \end{eqnarray*}
  For every node $i \in V_\text{OR}$ and every outgoing edge $(i, j) \in E$ we
  add a mode $m_{(i,j)}$ in $\M_G$ with the point-distribution to vector
  $\eta_{(i,j)}$. 
  For every node $i \in V_\text{AND}$ we add a mode $m_{i}$ in $\M_G$ with the
  uniform distribution over all vectors $\eta_{(i, j)}$ such that $(i, j) \in  E$.
  We next add the safety set:
  For every variable $x_i$ we add constraint $0 \leq  x_i \leq 1$ and  for every pair
  of variable $x_i, x_j$  such that $i \not = j$, we have $\neg((0 \leq x_i \leq 1) \wedge (0 \leq x_j
  \leq 1))$. 

  We show that for vertices $a, b \in V$ we have
  that $b$ is reachable from $a$ in graph $G$ iff $\vec{x}_b$ is reachable from
  $\vec{x}_a$ in the \smms{} $\M_G$ where $\vec{x}_i(j) = 1$ if $i = j$ and
  $\vec{x}_i(j) = 0$ otherwise.
  First we show that if node $b$ is reachable form node $a$ in graph $G$, the
  vertex $\vec{x}_b$ is reachable from the vertex $\vec{x}_a$ almost surely.
  There are three cases to consider.
  \begin{enumerate}
    \item
      $a = b$. In this case $\vec{x}_a = \vec{x}_b$ and hence the claim
      trivially follows. 
    \item
      $a \in V_\text{OR}$. Since $b$ is reachable form $a$, there must be a
      successor $a'$ of $a$ such that $b$ is reachable form $a$.
      Assuming that $\vec{x}_{a'}$  can reach $\vec{x}_b$ almost surely, we
      prove that $\vec{x}_{a}$  can reach $\vec{x}_b$ almost surely.
      Notice that is we choose mode $m_{(a,a')}$ for one time-unit, the system
      is safe during this time, and the variable $x_a$ decreases by $1$ and
      variable $x_{a'}$ increases by $1$ resulting in the state $\vec{x}_{a'}$.
      Hence, using inductive hypothesis, the
      vertex $\vec{x}_b$ is reachable from the vertex $\vec{x}_a$ almost surely.
    \item
      $a \in V_\text{AND}$. Since $b$ is reachable form $a$, all of the
      successors $a'$ of $a$ are such that $b$ is reachable form $a'$. 
      Assuming that all of the successors $a'$ of $a$  the state $\vec{x}_{a'}$
      can reach $\vec{x}_b$ almost surely, we 
      prove that $\vec{x}_{a}$  can reach $\vec{x}_b$ almost surely.
      Notice that is we choose mode $m_{a}$ for one time-unit, the system
      is safe during this time, and according to probability distribution one of
      the rate $\eta_{(a, a')}$ is given by the environment, and  the variable $x_a$
      decreases by $1$ and variable $x_{a'}$ increases by $1$ resulting in the
      state $\vec{x}_{a'}$. 
      Hence, using inductive hypothesis, vertex $\vec{x}_b$ is reachable from
      the vertex $\vec{x}_a$ almost surely.
  \end{enumerate}
  Now we prove the other direction by showing that
  if vertex $\vec{x}_b$ is reachable from the vertex $\vec{x}_a$ almost surely
  then node $b$ is reachable form node $a$ in graph $G$.
  Notice that he controller can suggest exactly one-unit of time delay in each
  mode since staying more than one time-unit will violate the safety condition
  $0 \leq x_i \leq 1$ for some variable $x_i$ and spending less than one
  time-unit will violate the condition $\neg ((0 \leq x_i \leq 1) \wedge (0 \leq
  j \leq 1))$ for some pair $i$ and $j$. 
  Given this restriction, the stochastic multi-mode system can be considered as
  a Markov decision process with states $\vec{x}_a$ for all $a \in V$ and we get
  that if it is possible to reach  vertex   $\vec{x}_b$ from $\vec{x}_a$ almost
  surely, it is possible to do so following positional strategies.
  Let us consider one such positional strategy that allows almost sure
  reachability.
  Note that from the starting vertex $\vec{x}_{a}$, from construction, we have
  that the system must choose
  either the mode $m_{(a,b'})$ if $a$ is an OR vertex, or the mode $m_{a}$
  if $a'$ is an AND vertex.
  The proof now follows from an easy inductive argument. 
\end{proof}


\subsection{Almost-Sure Discrete Reachability}
In this section we discuss almost-sure  {\em discrete reachability problem}, in which
the scheduler can only make decisions at integer multiples of a specified
\emph{clock period} $\Delta$ and every mode has only finitely many choices of rates.
%
Formally, given a \smms{} $\M$, a closed convex polytope $S$ as safety set, an
initial state $x_s \in S$, a target state $x_t \in S$, the discrete reachability
problem is to decide if there exists a schedule to reach $x_t$ from $x_s$
almost-surely where the time delays are multiples of $\Delta$.   

\begin{theorem}\label{thm:discr}
  Almost-sure discrete reachability problem is EXPTIME-complete.
\end{theorem}
\begin{proof}
  EXPTIME-membership of the problems is shown via discretization of the state
  space of $\M$.
  Since the set $S$ is given as a bounded polytope, the size of the
  discretization can be shown to be at most exponential in the size of $\M$
  and $\Delta$, and since the almost-sure reachability can be solved on Markov
  decision processes can be solved in P, EXPTIME-membership follows.

  The hardness is shown by a reduction from the countdown games~\cite{JLS08}. 
A countdown game is a tuple $\mathcal{G} = (N, T, n_1, B_1)$ where 
\begin{itemize}
\item
  $N = \set{n_1, n_2, \ldots, n_d}$ is a finite set of nodes;
  \item
    $T \subseteq N \times \Nat_{>0} \times N$ is a set of transitions; and
  \item
    $(n_1, B_1) \in N {\times} \Nat_{>0}$ is the initial configuration.
  \end{itemize}
  From any configuration $(n, B) \in N \times \Nat_{>0}$, 
  first player~1 chooses a number  $k \in \Nat_{>0}$, such that $k
  {\leq} B$ and there exists some $(n, k, n') \in T$, and then player~2
  chooses a transition $(n, k, n'') \in T$ labeled with that number. 
  Note that there can be more than one such transition.
  The new configuration then transitions to $(n'', B {-} k)$. 
  Player~1 wins a play of the game when a configuration $(n, 0)$ is
  reached, and loses (i.e., player~2 wins) when a configuration
  $(n, B)$ is reached in which player~1 is stuck, i.e., for all transitions
  $(n, k, n') \in T$, we have $k > B$.
  
  For a countdown game $(N, T, n_1, B_1)$ we define a \smms{} $\M$, a safety
  set $S$ and an initial state $\px_s$ and target state $\px_t$ such that there
  is a discrete schedule with $\Delta=1$ that reaches $\px_t$ a.s. if and only
  if player 1 has a winning strategy in the countdown game.   
  W.l.o.g we assume that when $(n, k, n')\in T$, then $n \neq n'$, and also we
  assume that the initial state is $(n_1, B_1)$ and there is no node $n$ and $k$
  such that $(n, k, n_1)\in T$. 

  The \smms{} $\M$ has $d+1$ variables. 
  The intuition is that the value of the first variable corresponds to the value
  of the counter, while $(i+1)$-th variable is equal to $1$ if the game is in
  node $n_i$, and $0$ otherwise. 
  
  For all $n, k \in N \times \Nat_{>0}$ such that there is $(n, k, n')\in T$ for
  some $n'$, we add a  mode $(n, k)$ to $\M$. 
  For all $(n_i, k, n_j)\in T$, we add the rate $r$ to the mode $(n_i, k)$
  such that the first component of $r$ is $-k$, the $(i+1)$-th component is
  $-1$ and $(j+1)$-th component is $1$. 
  All other components of $r$ are zero. 
  %% We further add modes $m_i$ for $3 \le i \le d+1$ which contain the unique rate
  %% with $B_1$ in the first component, $1$ in the second component, and $-1$ in
  %% $the i$-th component. 
  %% All other components of this rate are zero. 

  The safety set $S$ is defined so that the only points of $S$ with integer values are
  exactly $(i_1,\ldots, i_{d+1})$, where $0\le i_1\le B_1$, and exactly one of
  $i_2,\ldots, i_{d+1}$ is $1$, while the others are $0$. Such safety set can be
  defined using equations 
  \[
  \begin{array}{rl}
    x_1&\le B_1\\
    \sum_{i=2}^{d+1} x_i &\le 1\\
    x_i &\ge 0\qquad\text{for $1\le i\le d+1$}
  \end{array}
  \]
  and so in particular it is convex.
%  
  Now we claim that the system can reach $\px_t$ from $\px_s =
  (B_1,1,0,0,\ldots,0)$ almost-surely if and only if player 1 has a winning
  strategy in the countdown game. 
  The intuition is that the winning strategy for player 1 in the countdown game
  directly gives a strategy for the scheduler in $\M$ such that a point is
  reached which has zero in the first component, and zeros everywhere else
  except for some $i$-th component. 
%  Then the scheduler uses the mode $m_i$, which leads back to the initial state;
%  from there it uses the same strategy. 
  On the other hand, if player 2 has a winning strategy in the countdown game,
  this strategy can be used to get to a state from which the scheduler has no
  chance but to leave the safety set (which corresponds to not having any
  choices in the countdown game).  \qed
  % Note on the assumption: I think the assumption ``when $(s,\ell,s')\in T$, then
  % $s\neq s'$'' is required, because when simulating a step of the countdown
  % game, we need to be always removing 1 and adding 1 at two different
  % components. The assumption with $s_1$ not being on the rhs of any rule is
  % required for the modes returning to the start to work. 
\end{proof}

%could you please write this section on the computational
%   aspects of the proposed algorithm including a clean algorithm for
%   reachability, complexity of finding $\lambda$?} 
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% TeX-PDF-mode: t
%%% End:


==> explore.tex <==
\begin{figure*}[ht]
	\def\myscale{0.8}
	\centering
	\subfloat[]{\label{fig:movecentere}
		\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=0.5cm,
		semithick,scale=\myscale,every node/.style={transform shape}]
		%  \draw[shadowed={double=gray,draw=gray},fill=black!10,opacity=0.5] (0, 0)
		%  circle (2cm);
		\draw[] (0, 0) circle (2.5cm);
		\draw node (r1l) at (0.2,0.2) {$x_0$};
		\draw node (r2l) at (-0.25, -1.15) {$y_k$};
		\draw[-,dotted] (0, -1) -- node[below] {$\sqrt{\alpha(k)}$} (2.3, -1);
		\draw[dotted,->] (0, 0) -- node[right, pos=0.5] {$~~r$} (2.3, -1);
		\draw node (r1) at (0, 0) {};
		\draw node (r2) at (0, -1){};
		\draw[fill=black] (r1) circle(0.05);
		\draw[fill=black] (r2) circle(0.05);
		\draw[dotted] (0, 0) circle (0.5cm);
		
		\draw[-,dotted] (-3, 0) -- (3, 0);
		\draw[-,dotted] (0, -2.8) -- (0, 2.8);
		\end{tikzpicture}}%
	\subfloat[]{\label{fig:movecircle}
		\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=0.5cm,
		semithick,scale=\myscale,every node/.style={transform shape}]
		%  \draw[shadowed={double=gray,draw=gray},fill=gray!10,opacity=0.5] (0, 0) circle
		%  (2cm);
		\def\ra{0.4}
		\draw[] (0, 0) circle  (2.5cm);
		\draw node (r1l) at (-1.6, -0.7) {$x_s$};
		
		\draw node (r1) at (-1.6, -0.2) {};
		\draw[fill=black] (r1) circle(0.05);
		\draw[dashed] (r1) circle(\ra);
		
		\draw node (rdl) at (1.6, -0.7) {$x_t$};
		\draw node (rd) at (1.6,-0.2){};
		\draw[fill=black] (rd) circle(0.05);
		\draw[dashed] (rd) circle(\ra);
		
		
		\foreach \i in {0,...,8}
		{
			\draw node (\i) at (-1.6+\ra*\i, -0.2) {$u_{\i}$};
			\draw[fill=gray!30,color=gray] (\i) circle(0.05);
			\draw[dashed,color=gray] (\i) circle(\ra);
		}
		\draw[-,opacity=0.5,dotted] (-3, 0) -- (3, 0);
		\draw[-,opacity=0.5,dotted] (0, -2.8) -- (0, 2.8);
		\end{tikzpicture}}
	\subfloat[]{\label{fig:necessity}
		\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=0.5cm,
		semithick,scale=\myscale,every node/.style={transform shape}]
		\draw[-, color=black!20, dashed] (0,0) -- (-2.5,-2.5);
		\draw[->, color=black, thick] (0,0) -- (2.5,2.5);
		
		\draw[-,decorate,decoration={brace,amplitude=4pt,mirror,raise=1pt},yshift=0pt] (0.4,-0.4) -- node[below] {$~~~~~~\frac{\delta}{2}$} (1.5, 0.7);
		
		\draw[-,dotted] (-3, 0) -- (3, 0);
		\draw[-,dotted] (0, -2.8) -- (0, 2.8);
		
		\draw[->] (0, 0) -- (-2, -0.5);
		\draw[-,thick,color=black!30] (0, 0) -- node [color=black,right, pos=0.8] {$\alpha(k)$} (-1.3, -1.3);
		
		\draw node (r1l) at (-0.7,0.2) {$y(0)= x_s$};
		
		\draw node (yll) at (-2, -0.3) {$y(k)$};
		\draw node (y1) at (-2, -0.5) {};
		\draw node (r2l) at (1.2, 0.9) {$x_t$};
		\draw node (vl) at (2, 1.5) {$\vec{v}$};
		\draw node (r1) at (0, 0) {};
		\draw node (r2) at (1, 1){};
		\draw[fill=black] (r1) circle(0.05);
		\draw[fill=black] (r2) circle(0.05);
		\draw[dotted] (1, 1) circle (0.6cm);
		\draw[dotted,->] (1, 1) -- node[right, pos=0.7] {$~\frac{\delta}{4}$} (0.5, 1.5);
		\end{tikzpicture}}%\hspace{1em}
	\caption{Stochastic multi-mode system: proof sketch.\label{fig:smms-proof}}
\end{figure*}

==> s-t-reach.tex <==
\begin{figure*}[t]
\begin{center}
\scalebox{1}{
  \begin{tikzpicture}
    \draw (0, 0) circle (2cm);

  \draw node (r1l) at (1.5,0.3) {$x_t$};
  \draw node (r1) at (1.5, 0) {};
  \draw[fill=black] (r1) circle(0.05);
  \draw[] (r1) circle  (0.4);
  
  \draw node (r2l) at (-1.5, 0.3) {$x_s$};
  \draw node (r2) at (-1.5, 0){};
  \draw[fill=black] (r2) circle(0.05);
  \draw[fill=blue!60] (r2) circle  (0.4);
  
  \draw[-] (-3, 0) -- (3, 0);
  \draw[-] (0, -2.8) -- (0, 2.8);

  \draw[-] (r2) -- (r1);

  \draw[xshift=10pt, fill=black!55 ] (-1.5, 0) circle  (0.4);
  \draw[xshift=20pt, fill=black!50] (-1.5, 0) circle  (0.4);
  \draw[xshift=30pt, fill=black!45] (-1.5, 0) circle  (0.4);
  \draw[xshift=40pt, fill=black!40] (-1.5, 0) circle  (0.4);
  \draw[xshift=50pt, fill=black!35] (-1.5, 0) circle  (0.4);
  \draw[xshift=60pt, fill=black!30] (-1.5, 0) circle  (0.4);
  \draw[xshift=70pt, fill=black!25] (-1.5, 0) circle  (0.4);
  \draw[xshift=80pt, fill=black!20, fill opacity=0.2] (-1.5, 0) circle  (0.4);
  
%  \draw[color=gray, style=dotted] (-3, -3,0)
%  grid[xstep=1cm, ystep=1cm] (3, 3);

\end{tikzpicture}}
\caption{Stochastic multi-mode system: proof sketch.}
\label{fig:intro-example}
\end{center}
\end{figure*}

